Human-Robot Team Performance Compared to Full Robot Autonomy in 16 Real-World Search and Rescue Missions: Adaptation of the DARPA Subterranean Challenge

Human operators in human-robot teams are commonly perceived to be critical for mission success. To explore the direct and perceived impact of operator input on task success and team performance, 16 real-world missions (10 hrs) were conducted based on the DARPA Subterranean Challenge. These missions were to deploy a heterogeneous team of robots for a search task to locate and identify artifacts such as climbing rope, drills and mannequins representing human survivors. Two conditions were evaluated: human operators that could control the robot team with state-of-the-art autonomy (Human-Robot Team) compared to autonomous missions without human operator input (Robot-Autonomy). Human-Robot Teams were often in directed autonomy mode (70% of mission time), found more items, traversed more distance, covered more unique ground, and had a higher time between safety-related events. Human-Robot Teams were faster at finding the first artifact, but slower to respond to information from the robot team. In routine conditions, scores were comparable for artifacts, distance, and coverage. Reasons for intervention included creating waypoints to prioritise high-yield areas, and to navigate through error-prone spaces. After observing robot autonomy, operators reported increases in robot competency and trust, but that robot behaviour was not always transparent and understandable, even after high mission performance.

==> extendedabstract.tex <==
Operators in human-robot teams are commonly perceived to be critical for mission success in search and rescue expeditions. To explore the direct impact of operator involvement on mission performance, 16 real-world missions based on the DARPA Subterraran Challenge were tested to capture team performance metrics. Missions (10-hours total) involved using a heterogeneous robot team to navigate challenging terrain with the goal to locate as many items as possible, such as a rope, drill or survivor. Two conditions were evaluated: operators could directly control a robot team with state-of-the-art robot autonomy (Human-Robot Team Condition, CH) compared to observing autonomous mission execution by the robots without operator input (Robot Autonomy Condition, CA). Results found that Human-Robot Teams had an average tele-operation time of 2 minutes per mission (7.6\% of mission time), found more items (+8 items, +10.5\%), covered more unique ground (+5830 sq ft, +10.6\%), had a greater total distance (+3708 ft, +12.7\%) compared to robot autonomy alone. Human-Robot Teams were faster at finding the first item (-38 seconds, +23.3\%), but were slower to respond to information from the robot team (+70 seconds, -106\%). Human-Robot Teams used the robot eStop function fewer times (-9 uses, -54.5\%) and spent less time in eStop mode (-20 min, -47.62\%), representing fewer error-related events and faster recovery from error time. In optimal conditions, operator and autonomy-led scores were comparable in items found, distance travelled and unique coverage. In less predictable scenarios, operators were essential to high team performance, but at the expense of significant increases in cognitive load and perceived effort to lead the mission. Reasons for operator intervention included to speed up mission objectives, to cover more unique ground, to control robots through rough terrain areas, to prioritise high-yield areas, and to maintain tighter coordination efforts. Operators reported notable changes to perceived robot competency, trust in autonomous robot teams, and were less likely to intervene in future. However, operators reported that autonomous robot behaviour was not always clear and understandable, even after similar team performance scores. Overall, operators do improve team performance scores but can introduce delays in team coordination, which could be critical depending on how urgent or serious a 30-70 second delay to select the next robot action would represent for the mission. 

==> sparequalitativeinterview.tex <==
\subsection{Mission 1 - Course 1 - Human-Robot Team (FO)}
The following breakdown of Mission 1 is provided by the operator. 

\begin{displayquote} "As far as I can tell, there were no areas of the course that I missed, or that the robots missed" ... "It was pretty simple. The objects just kept coming in, and it was mostly easy to correctly score them.  The only trouble I had was with one object, which seemingly wasn't in the place that it thought it was, but I think we're tracking that up to an error on the scoring server side. "I think it [map coverage] was above 90 per cent.  Unless there's a sneaky area that I wasn't aware of, but yeah, it seemed really good. I didn't have to babysit the robots too much." [Mission 1, F, CB] \end{displayquote} 

\begin{displayquote} "I sent one of the ATRs to the left side of the course, and it did its thing and did really well. I sent the other ATR to the right side of the course, and it also did very well. It got stuck on the back hill a little bit, I'm not sure exactly why, and then I had one of the Spots come up, and it followed the first ATR and it filled in the gaps that the first ATR had missed. I did give it a little bit of direction in terms of sending the ATR to the far part of the course so that it wouldn't get close to a Spot.  So there was no clashing there.  Then at some point, I think the Spot had finished up everything it could do in that area, so I sent it back to follow the second titan on the other side of the course, and I don't think it quite got down there in time.  It might have done a little bit, and potentially if I had that fourth agent, I might have been able to send it down instead and been a bit more efficient.  But otherwise, it went pretty well. The time limit made it a little bit more difficult, as well as the reporting limit, but overall, the course was pretty easy from the robots' perspective, I would say" ... "I’m pretty happy with that.  It's a good first start." [Mission 1, F, CB] \end{displayquote} 

\begin{displayquote} There was an issue with the scoring server halfway through, where I was sending reports and they were coming back as errors. That was an error on the scoring server side, which was remedied, so that slowed me down a little bit, because I was sending reports and I was just getting errors back" [Mission 1, F, CB] \end{displayquote} 

\subsection{Mission 2 - Course 1 - Robot Autonomy (FO)}
The following breakdown of Mission 2 is provided by the operator. 

\begin{displayquote} "The first ATR decided to explore on the right side of the course" ... "The second ATR started up, did the same routine. It decided to explore into the tunnel to the left side of the course. It followed the first titan to the right side of the course.  Not too long after, it was trying to explore into some sort of grass area, and it fell down, and it was end of run. The other two ATRs did pretty well at exploring their sections of the course each and I would say got to the end of their respective sides and then started coming back. Then right towards the end, one of the ATRs got really close to a dangerous position, and we e-stopped it, and it was end of run for that ATR." ... "Overall, I'd say that in this run, we explored a little bit less than we did in the first run. There was maybe one or two sections that we didn't explore that we did in the first run." ... "They [Mission 1 and 2] were pretty similar as far as I could tell. I didn't see any changes"\end{displayquote} 

\subsection{Mission 3 - Course 1 - Human Robot Team (BO)}
The following breakdown of Mission 3 is provided by the operator. 

\begin{displayquote} "I think everything went pretty smoothly. There wasn't any catastrophes, didn't lose any robots. In most regards, they did what I told them to do, so there wasn't anything too out of the ordinary with regards to terrain difficulty. Mostly autonomous, as well, so there was a bit of directing at the start. Usually, the strategy is to split the robots up, send - I always like to use a pair, like a Spot and an ATR in one direction and a Spot and an ATR in the other direction.  So yeah, that all went well." ... "I think this was probably the easiest one I've done for a very long time." ... "Yeah, so terrain wise or coverage wise, I don't think I missed anything that the robots couldn't get through, so yeah, terrain wise was a fairly straightforward". "Those were really the only two times" in which the operator needed to intervene in the mission run but "otherwise, everything operated as expected." [Mission 3, B, CB] \end{displayquote} 

\subsection{Mission 4 - Course 1 - Robot Autonomy (BO)}
The following breakdown of Mission 4 is provided by the operator. 

\begin{displayquote} "We unfortunately had two Spots both get low battery warnings. They both did very well at covering, so obviously no intervention by me, but yeah, both - one in particular didn't make it to the end of the tunnel." An ATR "looked like it was going up, going down. There was plenty of room for it get through." ... "But otherwise, we got 13 things, which is really good". "If wasn't for the batteries and the precarious motor fault, I'm pretty confident the autonomy would have worked really well. The robots did a really good job of splitting themselves up, which is what you want." [Mission 4, B, CA] \end{displayquote} 

\subsection{Mission 5 - Course 2 - Human Robot Team (FO)}
The following breakdown of Mission 5 is provided by the operator. 

\begin{displayquote} One of the agents didn't start up initially on time, so I had to use the two ATRs. I sent one to the left-hand side of the course and one to the right-hand side of the course.  I think it was rat towards the barrels and bear towards the tunnel." ... "One of them got stuck near some barrels and I tele-oped it back a little bit just to free it, and similarly, for the other one in the tunnel was slipping on some part of the course and I had to push it into the tunnel." ... "Then the Spot became available, and I sent it in after bear into the tunnel. That was mainly to look underneath the landing.  It did a really good job exploring in there and found a very sneaky helmet under the landing. At that point, it followed up the titan and filled in the gaps between the - that the titan missed.  Meanwhile, rat had managed to get around behind S block and found a constriction in the form of a chair in the middle of the pathway, and it had a little bit of difficulty to get through that. It went through the first time, and then I left it alone, and then when I came back, it had come back past it again. So I had to force it again back past the chair, to keep looking in that direction" ... "Rat continued to go further along that part of the course and eventually got to a room, like a doorway to a room, which was quite tough for it, I think.  But it managed to get through all right and I think found an object.  At that point, I left it alone, because there wasn't much else for it to do, and I concentrated on the other two. I managed to - bear had managed to get itself into a dead end and was exploring a separate branch compared to Spot. So Spot, I managed to put Spot into the other branch, and it did a really good job of going to the other end of the tunnel and found an object, and then backtracked and did the same." ... "Some of the course - the course was a little bit more difficult and windy than I expected, but that's not too bad." [Mission 5, F, CB] \end{displayquote} 

\subsection{Mission 6 - Course 2 - Robot Autonomy (FO)}
The following breakdown of Mission 6 is provided by the operator. 

\begin{displayquote} 
"Started with – I want to say rat. Actually, no, it was bear first, and it went down to the barrel area, and then rat went into the tunnel area, and then finally [Chilli], which went - followed down to the barrels. Rat did a pretty good job in the tunnel initially, but eventually made its way outside and was unable to leave the outside the tunnel area via the secondary entrance further into the tunnel and just hung around doing not a lot, picking up some other frontiers. It eventually did explore under the landing in the cathedral, and it did find a helmet, but it did miss a good chunk of the tunnel course.  Bear, meanwhile, explored down to the barrels quite well, explored the barrels, found a couple of objects, got behind S block, but could not get past a chair constriction behind S block, and eventually made its way back up the hill and got stuck on a fence. Meanwhile, Chilli did almost nothing the entire run and just hung around the donga.  I don't even know if it scored any points at all." [Mission 6, F, CA] \end{displayquote} 

\subsection{Mission 7 - Course 2 - Human-Robot Team (BO)}
The following breakdown of Mission 7 is provided by the operator.

\begin{displayquote} "It was a much more stressful run than yesterday. So in general, the robots behaved very well, except I lost a Spot. It fell over, which changed my plans somewhat.  I had to get a titan from one end of the map to the other, and there was a lot more finicky terrain that I had to consider today compared to yesterday, which was fun as well. Yeah, it went well, but there was a lot more intervention by me, much more tele-ops and things like that." [Mission 7, B, CB] \end{displayquote} 

\subsection{Mission 8 - Course 2 - Robot Autonomy (BO)}
The following breakdown of Mission 8 is provided by the operator.

\begin{displayquote} "I think today's run was obviously a bit more complicated, so it was really good to see how the autonomy worked" ... "They split up, so two ATRs went in two different directions, which was good, and then the Spot wasted a bit of time gobbling up local frontiers, but yeah, they both - they covered the map very well autonomously and even did some pretty cool things getting through very narrow spaces, and always very well. [Mission 8, B, CA] \end{displayquote} 

\subsection{Mission 9 - Course 3 - Human Robot Team (FO)}
The following breakdown of Mission 9 is provided by the operator.

\begin{displayquote} "First I got Chilli up, I sent it down to the barrels, just because there were some constrictions down there, last time, that tripped up some robots, so I thought Chilli would be better to do that. I then sent - I can’t remember which one - I think it’s Rat, into the tunnel, it happily started exploring the tunnel, then sent Bear into the little playground next to donga, just because it was a bit difficult for Spot to do. Bear did a good job on the playground, got stuck once or twice, I had to sort of push it to get it - teleop it, push it via teleop to get it back on track. It quickly finished that to my satisfaction, so I deprioritised that region for all agents, then I sent Bear down to the barrels to help Chilli. Chilli, meanwhile, had had a quick look around the barrels, but not fully, and had gone behind S-Block and continued its way along S-Block.. Meanwhile, Rat had got into the tunnel, was doing a good job in the tunnel, had a couple of dead ends, but managed to make its way to the outside of the tunnel. Bear got down to the barrels, completed exploring the barrels, I feel like I didn’t get enough objects in the barrels, just based on how much space there is there, I may have missed something, but Bear did a good job exploring. Chilli, meanwhile, did a great job going all the way down to the [Gator] room, looked inside there, found an object in there. Bear, meanwhile, started to go behind S-Block to help Chilli, I figured Chilli didn’t need any help, instead there seemed to be an empty area in the tunnel, in the final section of the tunnel. I sent Bear all the way back up there to help out with that. Rat, meanwhile, was going up right to the back end of the tunnel, I think at that point I was reviewing objects, Rat completed its task all the way back to the end of the tunnel. Bear managed to get all the way to the tunnel in reasonably good time, I think that helped teleop it up the back row, just to speed it up, it looked in the [vinyl] section and found an object, which was good. Then, I think I let all the robots fill in the nooks and crannies, because by that point there was nothing left that was obvious to me to explore" [Mission 9, F, CB] \end{displayquote} 

\subsection{Mission 10 - Course 3 - Robot Autonomy (FO)}
The following breakdown of Mission 10 is provided by the operator.

\begin{displayquote} 
"I put it into autonomous mode and it went itself into the playground and did a pretty good job of exploring that. I then did Chilly, I think and Chilly decided to go down to the barrels and explore down the barrels. Then - I’ll turn this down. Then did Bear and Bear decided to go into the tunnel. Bear did a great job exploring the tunnel and sort of slowly made its way through every section except the [vinyl] section. Chilly, meanwhile, explored the barrels pretty well and then all behind S-block, W-block and X-block and I think covered everything, including the gator room. Then Rat decided to do pretty much nothing the entire run and explored various frontiers around the donga and then the back road. Then I think eventually it managed to find its way down to the barrels but really didn’t do a lot". [Mission 10, F, CA] \end{displayquote}

\subsection{Mission 11 - Course 3 - Human-Robot Team (BO)}
The following breakdown of Mission 11 is provided by the operator.

\begin{displayquote}
"The robots did really well, I split them up with my usual strategy, which was to send a Spot to go where I think it’ll go the deepest, and an ATR, on that split, a different way, then a third ATR which was exploring a local area. All those missions executed very well. No robots were lost in this mission, and I think we covered every nook and cranny of the course. Yeah, it was good" ... "No e-stops, no errors, no batteries, no fall overs" [Mission 11, B, CB] \end{displayquote} 

\subsection{Mission 12 - Course 3 - Robot Autonomy (BO)}
The following breakdown of Mission 12 is provided by the operator.

\begin{displayquote}
"The robots did very well. Explored every nook and cranny and detected every artefact. As far as I’m aware. So yeah, didn’t seem like any struggled. You know the Spot that went down to the barrels got into the smaller room very easily and the Titans that explored the tunnel did so very well. [Mission 12, B, CA] \end{displayquote} 

